Bayesian Reinforcement Learning: A Survey

Bayesian methods for machine learning have been widely investigated, yielding principled methods for incorporating prior information into inference algorithms. In this survey, we provide an in-depth review of the role of Bayesian methods for the reinforcement learning (RL) paradigm. The major incentives for incorporating Bayesian reasoning in RL are: 1) it provides an elegant approach to action-selection (exploration/exploitation) as a function of the uncertainty in learning; and 2) it provides a machinery to incorporate prior knowledge into the algorithms. We first discuss models and methods for Bayesian inference in the simple single-step Bandit model. We then review the extensive recent literature on Bayesian methods for model-based RL, where prior information can be expressed on the parameters of the Markov model. We also present Bayesian methods for model-free RL, where priors are expressed over the value function or policy class. The objective of the paper is to provide a comprehensive survey on Bayesian RL algorithms and their theoretical and empirical properties.

==> frontmatter.tex <==
%% Front matter for for FnT Machine Learning
%% (c) 2013 Neal Parikh (Stanford University)
%%
%% Based on earlier NOW style files by S. Kumar,
%% J. Sebastian, T. Hoekwater, and B.V. Elvenkind

\RequirePackage{lastpage}
\RequirePackage{multicol}

% base journal information definitions
\def\doi#1{\def\@doi{#1}}
\def\copyrightowner#1{\def\@copyrightowner{#1}}
\def\firstpage#1{\def\@firstpage{#1}}
\def\isbn#1{\def\@isbn{#1}}
\def\issue#1{\def\@issue{#1}}
\def\journalinfofont{\fontsize{8}{10}\selectfont\rmfamily}
\def\journallibraryinfo#1{\def\@libraryinfo{#1}}
\def\journaltitle#1{\def\@journaltitle{#1}}
\def\journaltitleprefix#1{\def\@journaltitleprefix{#1}}
\def\@lastpage{\pageref{LastPage}}
\def\lastpage#1{\def\@lastpage{#1}}
\def\copyrightyear#1{\def\@copyrightyear{#1}}
\edef\@copyrightyear{\the\year}
\def\pubyear#1{\def\@pubyear{#1}}
\edef\@pubyear{\the\year}
\def\volume#1{\def\@volume{#1}}

\def\journaltopicintro#1{\def\@journaltopicintro{#1}}
\def\journaltopics#1{\def\@journaltopics{#1}}

% editors
\newcount\editorcount
\def\@editors{}
\def\journaleditor#1{%
  \advance\editorcount1
  \ifx\empty\@editors
    \def\@editors{#1}%
  \else
    \expandafter\def\expandafter\@editors\expandafter{\@editors\\[0.3em]#1}%
  \fi
}

% editors in chief
\newcount\chiefeditorcount
\def\@chiefeditors{}
\def\journalchiefeditor#1{%
  \advance\chiefeditorcount1
  \ifx\empty\@chiefeditors
    \def\@chiefeditors{#1}%
  \else
    \expandafter\def\expandafter\@chiefeditors\expandafter{\@chiefeditors\\[0.3em]#1}%
  \fi
}

%% title page

\renewcommand\maketitle{\begin{titlepage}%

%\if@openright % -- for 'book' version
%\parindent \z@
%
%% title page
%\thispagestyle{empty}
%\vspace*{\fill}
%\begin{flushright}
%\begin{minipage}{0.8\textwidth}
%\begin{flushright}
%\renewcommand{\baselinestretch}{1.1}
%\sffamily\bfseries\huge
%\@title
%\end{flushright}
%\end{minipage}
%\end{flushright}
%\vspace*{\fill}
%
%% title+author page
%\cleardoublepage
%\thispagestyle{empty}
%
%\begin{flushright}
%{\renewcommand{\baselinestretch}{1.2}
%\sffamily\Huge\bfseries \@title\par}
%\vspace{3ex}
%\noindent\rule{\textwidth}{2pt}
%\vspace{1ex}\par
%
%\begingroup
%\def\and{%
%  \end{tabular}%
%  \par\vspace*{1.5ex}
%  \begin{tabular}[t]{r@{}}
%  \bfseries}
%
%  \fontsize{13}{15}\selectfont\sffamily
%\begin{tabular}[t]{r@{}}
%    \bfseries
%    \@author
%\end{tabular}
%\endgroup
%\vfill
%\includegraphics[width=53bp]{now_logo.pdf}\\
%\includegraphics[width=81bp]{essence_logo.pdf}\\
%Boston --- Delft
%\end{flushright}
%
%% publisher page
%\newpage
%\thispagestyle{empty}
%\begingroup
%
%\parskip6pt
%
%{\bfseries\sffamily\Large \@journaltitleprefix\ \@journaltitle}
%\footnotesize
%
%\vfill
%
%{\itshape Published, sold and distributed by:}\\
%now Publishers Inc.\\
%PO Box 1024\\
%Hanover, MA\ 02339\\
%United States\\
%Tel.\ +1-781-985-4510\\
%www.nowpublishers.com\\
%sales@nowpublishers.com
%
%{\itshape Outside North America:}\\
%now Publishers Inc.\\
%PO Box 179\\
%2600 AD Delft\\
%The Netherlands\\
%Tel.\ +31-6-51115274
%
%The preferred citation for this publication is
%
%{\raggedright
%\@copyrightowner. \emph{\@title}.  \@journaltitleprefix\
%\@journaltitle, vol.~\@volume, no.~\@issue, pp.~\@firstpage--\@lastpage,
%\@pubyear.\par}
%
%{\itshape This Foundations and Trends\textsuperscript{\textregistered} issue
%was typeset in \LaTeX\ using a class file designed by Neal Parikh. Printed on
%acid-free paper.}
%
%ISBN: \@isbn\\ \copyright\ \@copyrightyear\ \@copyrightowner
%
%\vfill
%
%\fontsize{8}{9}\selectfont
%All rights reserved. No part of this publication may be
%reproduced, stored in a retrieval system, or transmitted in any form
%or by any means, mechanical, photocopying, recording or otherwise,
%without prior written permission of the publishers.
%
%Photocopying. In the USA: This journal is registered at the Copyright
%Clearance Center, Inc., 222 Rosewood Drive, Danvers, MA 01923.
%Authorization to photocopy items for
%internal or personal use, or the internal or personal use of specific
%clients, is granted by now Publishers Inc for users registered with
%the Copyright Clearance Center (CCC).
%The `services' for users can be found on the internet at:
%www.copyright.com
%
%For those organizations that have been granted a photocopy license, a
%separate system of payment has been arranged. Authorization does not
%extend to other kinds of copying, such as that for general
%distribution, for advertising or promotional purposes, for creating
%new collective works, or for resale.  In the rest of the world:
%Permission to photocopy must be obtained from the copyright
%owner. Please apply to now Publishers Inc., PO Box 1024, Hanover, MA
%02339, USA; Tel. +1 781 871 0245; www.nowpublishers.com;
%sales@nowpublishers.com
%
%now Publishers Inc. has an exclusive license to publish this
%material worldwide. Permission to use this content must be obtained from
%the copyright license holder. Please apply to now Publishers, PO Box 179, 2600
%AD Delft, The Netherlands, www.nowpublishers.com; e-mail:
%sales@nowpublishers.com\par
%\endgroup
%
%% editorial board
%\newpage
%\thispagestyle{empty}
%\begin{center}
%\sffamily\LARGE
%{\bfseries \@journaltitleprefix\ \@journaltitle}\\
%{Volume \@volume, Issue \@issue, \@pubyear}\\
%{\bfseries Editorial Board}
%\end{center}
%
%\vspace{12pt}
%
%\ifnum\chiefeditorcount>1
%{\sffamily\bfseries Editors-in-Chief}
%{\footnotesize
%\begin{multicols}{2}
%\@chiefeditors
%\end{multicols}}
%\else
%{\sffamily\bfseries Editor-in-Chief}\par
%\vspace*{10pt}
%\begin{footnotesize}
%\begin{tabular}[t]{@{}l}
%\@chiefeditors \\
%\end{tabular}
%\end{footnotesize}
%\vspace*{10pt}
%\fi
%
%{\sffamily \bfseries Editors}
%{\footnotesize %\fontsize{9}{11}\selectfont
%\begin{multicols}{3}
%\raggedcolumns
%\@editors
%\end{multicols}}%
%
%% editorial scope
%\newpage % page vi -- blank
%\thispagestyle{empty}
%\begin{center}
%{\sffamily\bfseries\LARGE Editorial Scope}
%\end{center}
%
%\vspace{18pt}
%
%{\bfseries\large\sffamily Topics}\\
%
%\@journaltopicintro
%
%\fontsize{10}{13}\selectfont
%\begin{multicols}{2}
%    \raggedright
%    \@journaltopics
%\end{multicols}
%
%{\bfseries\large\sffamily Information for Librarians}\\
%
%\@libraryinfo\par
%
%\else\fi % -- no book front matter for "journal" version

% -- end book front matter

% title+author page
\newpage
\thispagestyle{empty}
\hbox to \textwidth{%
    \vbox{\raggedright
    \hsize=.6\textwidth \journalinfofont
{\hangindent=3.5ex
\hangafter=1
\@journaltitleprefix\ \@journaltitle\par}%
Vol.~\@volume, No.~\@issue\ (\@pubyear)
\@firstpage--\@lastpage\\
{\hangindent=3.5ex
\hangafter=1
\copyright\ \@copyrightyear\ \@copyrightowner\par}%
DOI: \@doi}\hss
\vbox{\hsize=.4\textwidth
    \raggedleft
    \includegraphics[width=53bp]{now_logo.pdf}\\
    \includegraphics[width=81bp]{essence_logo.pdf}\\
    \par
}}\par
\let\footnoterule\relax
\let\footnote\thanks
\null\vfil
\vskip 60\p@
\begin{center}%
{\LARGE \sffamily \bfseries \@title \par}%
\vskip 3em%
{
\large
\lineskip .75em%
     \lineskip .75em%
      \begin{tabular}[t]{c}%
        \@author
      \end{tabular}\par}%
\end{center}\par
\@thanks
\vfill
\end{titlepage}
\setcounter{footnote}{0}%
}

%% defaults and settings for this FnT

\def\@copyrightowner{now Publishers Inc.}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\volume{XX}
\issue{XX}
\firstpage{1}
\isbn{XXX-X-XXXXX-XXX-X}
\doi{10.1561/XXXXXXXXXX}

\journaltitle{Machine Learning}

\journalchiefeditor{\textbf{Michael Jordan} \\
University of California, Berkeley \\
United States}

\journaleditor{Peter Bartlett \\ \emph{UC Berkeley}}
\journaleditor{Yoshua Bengio \\ \emph{University of Montreal}}
\journaleditor{Avrim Blum \\ \emph{CMU}}
\journaleditor{Craig Boutilier \\ \emph{University of Toronto}}
\journaleditor{Stephen Boyd \\ \emph{Stanford University}}
\journaleditor{Carla Brodley \\ \emph{Tufts University}}
\journaleditor{Inderjit Dhillon \\ \emph{UT Austin}}
\journaleditor{Jerome Friedman \\ \emph{Stanford University}}
\journaleditor{Kenji Fukumizu \\ \emph{ISM, Japan}}
\journaleditor{Zoubin Ghahramani \\ \emph{University of Cambridge}}
\journaleditor{David Heckerman \\ \emph{Microsoft Research}}
\journaleditor{Tom Heskes \\ \emph{Radboud University} \columnbreak}
\journaleditor{Geoffrey Hinton \\ \emph{University of Toronto}}
\journaleditor{Aapo Hyvarinen \\ \emph{HIIT, Finland}}
\journaleditor{Leslie Pack Kaelbling \\ \emph{MIT}}
\journaleditor{Michael Kearns \\ \emph{UPenn}}
\journaleditor{Daphne Koller \\ \emph{Stanford University}}
\journaleditor{John Lafferty \\ \emph{University of Chicago}}
\journaleditor{Michael Littman \\ \emph{Brown University}}
\journaleditor{Gabor Lugosi \\ \emph{Pompeu Fabra University}}
\journaleditor{David Madigan \\ \emph{Columbia University}}
\journaleditor{Pascal Massart \\ \emph{University of Paris-Sud}}
\journaleditor{Andrew McCallum \\ \emph{UMass Amherst}}
\journaleditor{Marina Meila \\ \emph{University of Washington} \columnbreak}
\journaleditor{Andrew Moore \\ \emph{CMU}}
\journaleditor{John Platt \\ \emph{Microsoft Research}}
\journaleditor{Luc de Raedt \\ \emph{University of Freiburg}}
\journaleditor{Christian Robert \\ \emph{U Paris-Dauphine}}
\journaleditor{Sunita Sarawagi \\ \emph{IIT Bombay}}
\journaleditor{Robert Schapire \\ \emph{Princeton University}}
\journaleditor{Bernhard Schoelkopf \\ \emph{MPI T\"{u}bingen}}
\journaleditor{Richard Sutton \\ \emph{University of Alberta}}
\journaleditor{Larry Wasserman \\ \emph{CMU}}
\journaleditor{Bin Yu \\ \emph{UC Berkeley}}

\journaltopicintro{\@journaltitleprefix\ \@journaltitle\ publishes
survey and tutorial articles on the theory, algorithms and applications of machine learning, including the following topics:}

\journaltopics{
\begin{itemize}
\item{Adaptive control and signal processing}
\item{Applications and case studies}
\item{Behavioral, cognitive, and neural learning}
\item{Bayesian learning}
\item{Classification and prediction}
\item{Clustering}
\item{Data mining}
\item{Dimensionality reduction}
\item{Evaluation}
\item{Game theoretic learning}
\item{Graphical models}
\item{Independent component analysis}
\item{Inductive logic programming}
\item{Kernel methods}
\item{Markov chain Monte Carlo}
\item{Model choice}
\item{Nonparametric methods}
\item{Online learning}
\item{Optimization}
\item{Reinforcement learning}
\item{Relational learning}
\item{Robustness}
\item{Spectral methods}
\item{Statistical learning theory}
\item{Variational inference}
\item{Visualization}
\end{itemize}
}

\journallibraryinfo{%
  Foundations and Trends\textsuperscript{\textregistered} in \@journaltitle, \@pubyear,
  Volume~\@volume, 6 issues. ISSN paper version 1935-8237.
  ISSN online version 1935-8245.
  Also available as a combined paper and online
  subscription.
}

\endinput

